Leveraging Multilingual News Websites for Building a Kurdish Parallel Corpus

Machine translation has been a major motivation of development in natural language processing. Despite the burgeoning achievements in creating more efficient machine translation systems thanks to deep learning methods, parallel corpora have remained indispensable for progress in the field. In an attempt to create parallel corpora for the Kurdish language, in this paper, we describe our approach in retrieving potentially-alignable news articles from multi-language websites and manually align them across dialects and languages based on lexical similarity and transliteration of scripts. We present a corpus containing 12,327 translation pairs in the two major dialects of Kurdish, Sorani and Kurmanji. We also provide 1,797 and 650 translation pairs in English-Kurmanji and English-Sorani. The corpus is publicly available under the CC BY-NC-SA 4.0 license.

==> minutes.tex <==
25/04/2020: Dr. Hassani to ask the news agencies if they can provide the data with us



http://www.world-newspapers.com/kurdistan.html
http://www.nrttv.com/BA/News.aspx?id=21286&MapID=1
http://www.nrttv.com/News.aspx?id=30247&MapID=1

https://kurdpa.net



\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{coling2020/images/news_articles.pdf}
    \caption{A potentially identical news articles in Kurmanji (left) and Sorani (right). Corresponding sections are labelled similarly.}
    \label{fig_news_article}
\end{figure}


Kurdish is a complex member of Iranian languages.It includes several dialects each with various sub-dialects. Some of these dialects are not only mutually intelligible but also differ in the grammatical aspects \cite{hassani2016automatic}. The classification of these dialects still is a subject for scholarly debate. The two widely spoken dialects are usually referred to as Kurmanji and Sorani though the linguistic classification terms are different \cite{hassani2018blark,matras2019revisiting}. Kurdish is written in several scripts, but for the Kurmanji dialect the Latin script is more popular while Sorani is mostly written in the Arabic-Persian script. 

In order to support this hypothesis, we carried out an analysis on two basic dictionaries of Kurmanji-English and Sorani-English \cite{ahmadi2019lex} where we counted the number of lexical entries with identical translations in English. As both resources are in Latin script, no conversion of the scripts was required. Our analysis shows that among X\% headwords in the both dictionaries, X\% are written identically and have the same translations in English. In addition, X\% of the headwords exist in both dictionaries but translated differently. 


In this approach, we rely on the structure of the news articles in providing key information. For instance, Figure \ref{fig_news_article} illustrates two news articles from Rûdaw news website\footnote{https://www.rudaw.net}, in Sorani (right) and Kurmanji (left). Although the content of the two articles is almost identical, the content cannot be aligned systematically. In other words, there is no implicit link between the two news articles. However, the two articles are published in the same day with similar tags. % Sina: change this news article to one in ANF


\begin{table}[h]
\begin{tabular}{|l|l|l|l|l|}
\hline
Corpus                         & \# Aligned headlines & \# Aligned sentences & \# Word Tokens & \# Word types \\ \hline
\multirow{2}{*}{Kurmanji-Sorani} & \multirow{2}{*}{}    & \multirow{2}{*}{}    &                &               \\ %\cline{4-5} 
                                 &                      &                      &                &               \\ \hline
\multirow{2}{*}{Kurdish-English}                  & \multirow{2}{*}{}    & \multirow{2}{*}{}    &                &               \\% \cline{4-5} 
                                 &                      &                      &                &               \\ \hline
\end{tabular}
\caption{Basic statistics of the parallel corpora. Kurdish refers to the Kurmanji-Sorani translation pairs}
\label{tab_basic_stats}
\end{table}


\subsection{Quantitative analysis}
\subsection{Qualitative analysis}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 & \multicolumn{2}{l|}{}                   & kmr-eng                  & ckb-eng  & ckb-kmr  \\ \hline
 &                             & images    & 292/132                  & 143/70   & 917/507  \\ \cline{3-6} 
 &                             & headlines & 7472/71                  & 7113/142 & 3088/266 \\ \cline{3-6} 
 & \multirow{-3}{*}{Retrieved} & all       & 203                      & 212      & 773      \\ \cline{2-6} 
\multirow{-4}{*}{ANF} & \multicolumn{2}{l|}{Crawled}            & \multicolumn{3}{l|}{3026 (kmr) - 2432 (ckb) - 2937 (eng)}                      \\ \hline
                      &                             & images    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} \\ \cline{3-6} 
                      &                             & headlines & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 3144/129                 \\ \cline{3-6} 
                      & \multirow{-3}{*}{Retrieved} & all       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 129                      \\ \cline{2-6} 
\multirow{-4}{*}{BN}  & \multicolumn{2}{l|}{Crawled}            & \multicolumn{3}{l|}{1177 (kmr) - 1277 (ckb) - 701 (eng)}                       \\ \hline
 &                             & images    & 74/74                    & 75/70    & 188/135  \\ \cline{3-6} 
 &                             & headlines & \cellcolor[HTML]{C0C0C0} & 6300/10  &          \\ \cline{3-6} 
 & \multirow{-3}{*}{Retrieved} & all       & 74                       & 80       &          \\ \cline{2-6} 
\multirow{-4}{*}{KP}  & \multicolumn{2}{l|}{Crawled}            & \multicolumn{3}{l|}{663 (kmr) - 1281 (ckb) - 566 (eng)}                        \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}
